Generative Fractional Diffusion Models

We introduce the first continuous-time score-based generative model that leverages fractional diffusion processes for its underlying dynamics. Although diffusion models have excelled at capturing data distributions, they still suffer from various limitations such as slow convergence, mode-collapse on imbalanced data, and lack of diversity. These issues are partially linked to the use of light-tailed Brownian motion (BM) with independent increments. In this paper, we replace BM with an approximation of its non-Markovian counterpart, fractional Brownian motion (fBM), characterized by correlated increments and Hurst index $H \in (0,1)$, where $H=0.5$ recovers the classical BM. To ensure tractable inference and learning, we employ a recently popularized Markov approximation of fBM (MA-fBM) and derive its reverse-time model, resulting in generative fractional diffusion models (GFDM). We characterize the forward dynamics using a continuous reparameterization trick and propose augmented score matching to efficiently learn the score function, which is partly known in closed form, at minimal added cost. The ability to drive our diffusion model via MA-fBM offers flexibility and control. $H \leq 0.5$ enters the regime of rough paths whereas $H>0.5$ regularizes diffusion paths and invokes long-term memory. The Markov approximation allows added control by varying the number of Markov processes linearly combined to approximate fBM. Our evaluations on real image datasets demonstrate that GFDM achieves greater pixel-wise diversity and enhanced image quality, as indicated by a lower FID, offering a promising alternative to traditional diffusion models

==> tables/compute.tex <==
\begin{table}[t]
\centering
\begin{subtable}{.49\textwidth}
\scalebox{0.7}{
    \begin{tabular}{c|c c c | c |}
          &  $H=0.9$ & $H=0.5$ & $H=0.1$ & average \\  
         \hline
        VP &  - & \footnotesize{$0.0478$}\tiny{$\pm 0.1688$} & - & \footnotesize{$0.0478$} \\
        $K=1$ & \footnotesize{$0.0475$}\tiny{$\pm 0.0899$}  & \footnotesize{$0.0475$}\tiny{$\pm 0.0938$} & \footnotesize{$0.0475$}\tiny{$\pm 0.0900$} & \footnotesize{$0.0475$} \\ 
        $K=2$ & \footnotesize{$0.0476$}\tiny{$\pm 0.0907$}  & \footnotesize{$0.0477$}\tiny{$\pm 0.0917$} & \footnotesize{$0.0481$}\tiny{$\pm 0.0907$} & \footnotesize{$0.0478$} \\ 
        $K=3$ & \footnotesize{$0.0483$}\tiny{$\pm 0.0937$}  & \footnotesize{$0.0477$}\tiny{$\pm 0.0909$} & \footnotesize{$0.0477$}\tiny{$\pm 0.0950$} & \footnotesize{$0.0479$}\\ 
        $K=4$ & \footnotesize{$0.0476$}\tiny{$\pm 0.0899$}  & \footnotesize{$0.0479$}\tiny{$\pm 0.0916$} & \footnotesize{$0.0484$}\tiny{$\pm 0.0937$} & \footnotesize{$0.0480$}\\ 
        $K=5$ & \footnotesize{$0.0484$}\tiny{$\pm 0.0942$}  & \footnotesize{$0.0479$}\tiny{$\pm 0.0925$} & \footnotesize{$0.0479$}\tiny{$\pm 0.0930$} & \footnotesize{$0.0481$}\\ 
    \end{tabular}
    }
    \caption{Average training time in seconds}
\end{subtable}
\begin{subtable}{.49\textwidth}
\scalebox{0.7}{
    \begin{tabular}{c|c c c |  c |}
          &  $H=0.9$ & $H=0.5$ & $H=0.1$ & average \\  
         \hline
        VP &  - & \footnotesize{$2.3013$}\tiny{$\pm 0.1511$} & - & \footnotesize{$2.3013$}\\
        $K=1$  &  \footnotesize{$2.3036$}\tiny{$\pm 0.1290$} & \footnotesize{$2.3120$}\tiny{$\pm 0.1062$} & \footnotesize{$2.3031$}\tiny{$\pm 0.1133$} & \footnotesize{$2.3062$} \\
        $K=2$ &  \footnotesize{$2.3139$}\tiny{$\pm 0.1166$} & \footnotesize{$2.3070$}\tiny{$\pm 0.1102$} & \footnotesize{$2.3154$}\tiny{$\pm 0.1555$} & \footnotesize{$2.3121$} \\
        $K=3$ &  \footnotesize{$2.3134$}\tiny{$\pm 0.1246$} & \footnotesize{$2.3168$}\tiny{$\pm 0.1056$} & \footnotesize{$2.3309$}\tiny{$\pm 0.1096$} & \footnotesize{$2.3204$} \\
        $K=4$ &  \footnotesize{$2.3199$}\tiny{$\pm 0.1109$} & \footnotesize{$2.3091$}\tiny{$\pm 0.1132$} & \footnotesize{$2.3210$}\tiny{$\pm 0.1383$} & \footnotesize{$2.3167$} \\
        $K=5$ &  \footnotesize{$2.6568$}\tiny{$\pm 0.0984$} & \footnotesize{$2.6603$}\tiny{$\pm 0.0978$} & \footnotesize{$2.6692$}\tiny{$\pm 0.0975$} & \footnotesize{$2.6621$} \\
    \end{tabular}
}
\caption{Average sampling time in seconds}
\end{subtable}
\caption{Computational cost of GFDM compared to traditional diffusion models. (a) Average time in seconds for one training step with FVP dynamics on CIFAR10 with a batch size of $128$, a conditional UNet with $58.7mio$ parameters and EMA. (b) Average time in seconds for one sampling step in the reverse dynamics of FVP to generate data of dimension $(3,32,32)$ with a batch size of $1000$ using a conditional UNet with $58.7mio$ parameters with EMA for the score-model.}
\label{tab:compute}
\end{table}

==> tabletemplates/mini-tables.tex <==
\begin{table}[tb]
  \caption{\textit{Left:} Quantitative Results for the swiss roll dataset. Note that for $H=0.5$ the noisy ODE sampling (nODE) is equivalent to ODE sampling. \textit{Right:} Quantitative Results for the two moons dataset. Note that for $H=0.5$ the noisy ODE sampling (nODE) is equivalent to ODE sampling.}
  \label{tab:experiment-results:swiss-roll}
  \centering
  % default is 6, setting to 5
  \setlength{\tabcolsep}{3.5pt}
  \scalebox{0.5}{
  \begin{small}
      \begin{tabular}{ll lllll lllll lllll}
        \toprule
        % HEADING: the metrics
            &\multirow{2}{*}{$H$}
            & \multicolumn{3}{c}{WSD} & 
               \multicolumn{3}{c}{Impr. Prec} & 
               \multicolumn{3}{c}{Impr. Rec.} & 
               \multicolumn{3}{c}{Vendi} & 
               \multicolumn{3}{c}{NLL} \\
        \cmidrule(r){3-17}
        % SUBHEADING: FVP, Sub FVP & VE as scenarios for every metric
            && \scriptsize FVP & \scriptsize S.FVP & \scriptsize VE 
             & \scriptsize FVP & \scriptsize S.FVP & \scriptsize VE 
             & \scriptsize FVP & \scriptsize S.FVP & \scriptsize VE 
             & \scriptsize FVP & \scriptsize S.FVP & \scriptsize VE 
             & \scriptsize FVP & \scriptsize S.FVP & \scriptsize VE 
            \\
        \midrule
        % ROWS: different values for H (0.01, 0.25, 0.5)
        % TODO: Calculate the metrics and add the value into the placeholder "0.00"
        % --- SDE ---
        \multirow{3}{*}{\rotatebox{90}{SDE}}
        % H = 0.01
        & 0.01 & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % H = 0.25
        & 0.25 & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % H = 0.5
        & 0.5  & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % --- guided SDE ---
        \multirow{3}{*}{\rotatebox{90}{gSDE}}
        % H = 0.01
        & 0.01 & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % H = 0.25
        & 0.25 & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % H = 0.5
        & 0.5  & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % % --- ODE ---
        % \multirow{3}{*}{\rotatebox{90}{ODE}}
        % % H = 0.01
        % & 0.01 & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % % H = 0.25
        % & 0.25 & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % % H = 0.5
        % & 0.5  & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % --- noisy ODE ---
        \multirow{3}{*}{\rotatebox{90}{nODE}}
        % H = 0.01
        & 0.01 & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % H = 0.25
        & 0.25 & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % H = 0.5
        & 0.5  & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        \bottomrule
      \end{tabular}

      \begin{tabular}{ll lllll lllll lllll}
        \toprule
        % HEADING: the metrics
            &\multirow{2}{*}{$H$}
            & \multicolumn{3}{c}{WSD} & 
               \multicolumn{3}{c}{Impr. Prec} & 
               \multicolumn{3}{c}{Impr. Rec.} & 
               \multicolumn{3}{c}{Vendy} & 
               \multicolumn{3}{c}{NLL} \\
        \cmidrule(r){3-17}
        % SUBHEADING: FVP, Sub FVP & VE as scenarios for every metric
            && \scriptsize FVP & \scriptsize S.FVP & \scriptsize VE 
             & \scriptsize FVP & \scriptsize S.FVP & \scriptsize VE 
             & \scriptsize FVP & \scriptsize S.FVP & \scriptsize VE 
             & \scriptsize FVP & \scriptsize S.FVP & \scriptsize VE 
             & \scriptsize FVP & \scriptsize S.FVP & \scriptsize VE 
            \\
        \midrule
        % ROWS: different values for H (0.01, 0.25, 0.5)
        % TODO: Calculate the metrics and add the value into the placeholder "0.00"
        % --- SDE ---
        \multirow{3}{*}{\rotatebox{90}{SDE}}
        % H = 0.01
        & 0.01 & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % H = 0.25
        & 0.25 & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % H = 0.5
        & 0.5  & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % --- guided SDE ---
        \multirow{3}{*}{\rotatebox{90}{gSDE}}
        % H = 0.01
        & 0.01 & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % H = 0.25
        & 0.25 & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % H = 0.5
        & 0.5  & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % % --- ODE ---
        % \multirow{3}{*}{\rotatebox{90}{ODE}}
        % % H = 0.01
        % & 0.01 & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % % H = 0.25
        % & 0.25 & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % % H = 0.5
        % & 0.5  & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
        %          0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % --- noisy ODE ---
        \multirow{3}{*}{\rotatebox{90}{nODE}}
        % H = 0.01
        & 0.01 & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % H = 0.25
        & 0.25 & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        % H = 0.5
        & 0.5  & 0.00 &  0.00 &  0.00 &  % WSD (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Prec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Impr. Rec. (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 &  % Vendy (FVP, S. FVP, VE)
                 0.00 &  0.00 &  0.00 \\ % NLL (FVP, S. FVP, VE)
        \bottomrule
      \end{tabular}
  \end{small}
  }
  % default is 6, setting back to 6
  \setlength{\tabcolsep}{6pt}
\end{table}

==> tabletemplates/normal-tables.tex <==
\begin{table}[tb]
  \centering
  \caption{Quantitative results for the swiss roll dataset.} 
  \label{tab:experiment-results:swiss-roll}
  % default is 6, setting to 5
  \setlength{\tabcolsep}{6pt}
    % ---------------------------------
    % ---------- SWISS ROLL -----------
    % ---------------------------------
      \begin{scriptsize}
          \hspace{-0.25cm} % shift the table to the left by 0.25 cm
          \begin{tabular}{ll ll ll ll ll }
            \toprule
            % HEADING: the metrics
                &\multirow{2}{*}{$H$}
                & \multicolumn{2}{c}{WSD $\downarrow$} & 
                   \multicolumn{2}{c}{IP $\uparrow$} & 
                   \multicolumn{2}{c}{IR $\uparrow$} & 
                   \multicolumn{2}{c}{VS $\uparrow$} \\
            \cmidrule(r){3-10}
            % SUBHEADING: FVP, Sub FVP & VE as scenarios for every metric
                && \scriptsize FVP & \scriptsize S.FVP
                 & \scriptsize FVP & \scriptsize S.FVP
                 & \scriptsize FVP & \scriptsize S.FVP
                 & \scriptsize FVP & \scriptsize S.FVP 
                 % & \scriptsize FVP & \scriptsize S.FVP 
                \\
            \midrule
            % ROWS: different values for H (0.01, 0.25, 0.5)
            % TODO: Calculate the metrics and add the value into the placeholder "0.00"
            % --- SDE ---
            \multirow{2}{*}{\rotatebox{90}{SDE}}
            % H = 0.01 (SWISS ROLL & SDE)
            & 0.01 & \textbf{0.018} &  \textbf{0.020} &   % WSD (FVP, S. FVP)
                     0.614 &  0.955 &   % Impr. Prec. (FVP, S. FVP)
                     \textbf{0.993} &  \textbf{0.975} &   % Impr. Rec. (FVP, S. FVP)
                     \textbf{1.999} &  1.998 \\  % Vendi (FVP, S. FVP)
            % H = 0.25 (SWISS ROLL & SDE)
            & 0.25 & 0.020 &  0.022 &  % WSD (FVP, S. FVP)
                     0.705 &  0.953 &  % Impr. Prec. (FVP, S. FVP)
                     0.990 &  0.973 &  % Impr. Rec. (FVP, S. FVP)
                     \textbf{1.999} &  1.998 \\ % Vendi (FVP, S. FVP)
            % H = 0.5 (SWISS ROLL & SDE)
            & 0.5  & 0.021 &  0.027 &   % WSD (FVP, S. FVP)
                     0.871 &  0.967 &   % Impr. Prec. (FVP, S. FVP)
                     0.983 &  0.965 &   % Impr. Rec. (FVP, S. FVP)
                     \textbf{1.999} &  1.997 \\  % Vendi (FVP, S. FVP)
            % --- guided SDE ---
            \multirow{2}{*}{\rotatebox{90}{gSDE}}
            % H = 0.01 (SWISS ROLL & guided SDE)
            & 0.01 & 0.061 &  0.063 &  % WSD (FVP, S. FVP)
                     0.602 &  0.969 &  % Impr. Prec. (FVP, S. FVP)
                     0.991 &  0.960 &  % Impr. Rec. (FVP, S. FVP)
                     1.997 &  1.997 \\ % Vendi (FVP, S. FVP)
            % H = 0.25 (SWISS ROLL & guided SDE)
            & 0.25 & 0.053&  0.053&  % WSD (FVP, S. FVP)
                     0.703 &  0.964  &  % Impr. Prec. (FVP, S. FVP)
                     0.991 &  0.966 &  % Impr. Rec. (FVP, S. FVP)
                     1.997 &  1.998 \\  % Vendi (FVP, S. FVP)
            % H = 0.5 (SWISS ROLL & guided SDE)
            & 0.5  & - &  - & % WSD (FVP, S. FVP)
                     - &  - & % Impr. Prec. (FVP, S. FVP)
                     - &  - & % Impr. Rec. (FVP, S. FVP)
                     - &  - \\% Vendi (FVP, S. FVP, VE)
            % --- noisy ODE ---
            \multirow{2}{*}{\rotatebox{90}{nODE}}
            % H = 0.01 (SWISS ROLL & noisy ODE)
            & 0.01 & 0.126 &  0.135 &  % WSD (FVP, S. FVP)
                     0.968 &  0.985 &   % Impr. Prec. (FVP, S. FVP)
                     0.951 &  0.941 &  % Impr. Rec. (FVP, S. FVP)
                     1.986 &  1.988 \\  % Vendi (FVP, S. FVP)
            % H = 0.25 (SWISS ROLL & noisy ODE)
            & 0.25 & 0.162 &  0.172 & % WSD (FVP, S. FVP, VE)
                     \textbf{0.983} &  \textbf{0.992} & % Impr. Prec. (FVP, S. FVP, VE)
                     0.920 &  0.913 & % Impr. Rec. (FVP, S. FVP, VE)
                     1.979 &  1.968 \\ % Vendi (FVP, S. FVP, VE)
            % H = 0.5 (SWISS ROLL & noisy ODE)
            & 0.5  & 0.020 &  \textbf{0.020} &  % WSD (FVP, S. FVP)
                     0.940 &  0.964 & % Impr. Prec. (FVP, S. FVP)
                     0.971 &  0.970 & % Impr. Rec. (FVP, S. FVP)
                     \textbf{1.999} &  \textbf{2.00} \\% Vendi (FVP, S. FVP)
            \bottomrule
          \end{tabular}
      \end{scriptsize}
  % default is 6, setting back to 6
  \setlength{\tabcolsep}{6pt}
  \vspace{-.2cm}
\end{table}
